OpenREAD: Reinforced Open-Ended Reasoning for End-to-End Autonomous Driving with LLM-as-Critic

Recently, two-stage fine-tuning strategies, e.g., acquiring essential driving knowledge through supervised fine-tuning (SFT) and further enhancing decision-making and planning via reinforcement fine-tuning (RFT), have shown strong potential in advancing the knowledge-driven autonomous driving (AD) paradigm. However, the learning nature of SFT still limits the generalization of reasoning, thereby constraining the full potential of driving performance. Meanwhile, current RFT approaches are primarily applied to downstream tasks, since scene understanding is an open-ended problem where corresponding rewards are difficult to quantify. To address these limitations, we propose OpenREAD, an OPEN-ended REasoning reinforced vision-language model (VLM)-based autonomous driving (AD) framework that enables end-to-end RFT across the full spectrum from high-level reasoning to low-level trajectory planning. Specifically, we begin by constructing large-scale Chain-of-Thought (CoT) annotations on open-source driving-related knowledge datasets, and employ the powerful Qwen3 large language model (LLM) as the critic in RFT to quantify reasoning quality for open-ended questions during reward modeling. Extensive experiments confirm that joint end-to-end RFT yields substantial improvements in both upstream and downstream tasks, enabling OpenREAD to achieve state-of-the-art performance on reasoning and planning benchmarks.

==> sec/final_copy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/teaser.tex <==
% \begin{figure*}[!h]
% \centering
% % \includegraphics[width=0.5\textwidth %height=0.5\textwidth
% % ]{figs}
% \includegraphics[width=0.8\textwidth]{figs/teaser.pdf}
% \caption{\textbf{An overview of our \OURS}, a specialized vision-language model for end-to-end autonomous driving with extensive fundamental driving knowledge. Given a clip of the video sequence, our \OURS is capable of answering various driving-related questions and planning a trajectory according to the target waypoint.}
% \label{fig:teaser}
% \end{figure*}



==> tables/knowledge_ablation.tex <==
\begin{table*}[ht]
    \centering
    \setlength\tabcolsep{6pt}
    \renewcommand\arraystretch{1.2}
    \begin{tabular}{l|c|c|c|c|c|c|c|c|c} \hline
    \multirow{2}{*}{Dataset} & \multicolumn{3}{c|}{LingoQA$\uparrow$} & \multicolumn{2}{c|}{BDDX-Action$\uparrow$} & \multicolumn{2}{c|}{DriveLM-Obj$\uparrow$} & \multicolumn{2}{c}{HAD-Attention$\uparrow$}  \\ \cline{2-10}
    & L-Judge & BLEU & CIDEr & BLEU & METEOR & BLEU & METEOR & BLEU & METEOR  \\ \hline
    Carla & 13.4 & 2.2 & 21.5 & 0.0 & 2.2 & 4.4 & 4.0 & 0.0 & 0.2 \\ \hline
    Carla+LingoQA & 58.2 & 13.7 & 64.3 & 0.3 & 3.5 & 16.9 & 14.9 & 0.8 & 5.9 \\ \hline 
    \begin{tabular}{@{}l@{}@{}}Carla+LingoQA \\ +DRAMA \end{tabular} & \textbf{60.4} & \textbf{14.2} & \textbf{68.3} & \textbf{1.5} & \textbf{10.8} & \textbf{16.9} & \textbf{15.5} & \textbf{0.9} & \textbf{6.1} \\ \hline

    % C+L+DS & 58.4 & 13.5 & 61.4 & 0.0 & 2.8 & 9.4 & 12.6 & 0.8 & 5.4\\ \hline
    % C+L+DS+DR & \textbf{60.4} & \textbf{14.2} & \textbf{68.3} & \textbf{1.5} & \textbf{10.8} & \textbf{16.9} & \textbf{15.5} & \textbf{0.9} & \textbf{6.1} \\ \hline
    \end{tabular}
    % \begin{tabular}{c|c|c|c|c|c} \hline
    % \multirow{2}{*}{Dataset} & \multicolumn{2}{c|}{HPatches} & \multicolumn{2}{c|}{ETH3D} & KITTI \\ \cline{2-6}
    % & AEPE & PCK-1 & AEPE & PCK-1 & F1\\ \hline
    % C+T & 55.3 & 38.3 & 3.9 & 55.0 & 13.9 \\ \hline
    % M & 24.9 & 44.8  & 2.2 & 50.6 & 18.4 \\ \hline
    % M+Sc & 15.3 & 42.8 & \textbf{2.0} & 54.1 & 17.7\\ \hline
    % M+Sc+T+TA & \textbf{13.1} & 44.3 & \textbf{2.0} & 55.9 & 10.8  \\ \hline
    % M+Sc+T+TA+TS & 13.3 & \textbf{46.3}  & \textbf{2.0} & \textbf{56.3} & \textbf{9.6} \\ \hline
    % \end{tabular}
    \caption{Experiment on the effectiveness of extending training data on knowledge evaluation. C, L, D are short for Carla, LingoQA, DRAMA datasets, respectively. The best performance is reported in \textbf{bold}.}\label{tab:knowledge_ablation}
    \vspace{1mm}
\end{table*}
\vspace{-1mm}

==> tables/knowledge_eval.tex <==
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{4pt}
\caption{Comparison with existing methods on motion planning benchmarks. $\downarrow$ indicates lower is better.}
\begin{tabular}{lccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{VLM-Based}} & \multicolumn{2}{c}{\textbf{Ego Status}} & \multicolumn{4}{c}{$\mathbf{L2\ (m)\downarrow}$} & \multicolumn{4}{c}{\textbf{Collision (\%)$\downarrow$}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-8} \cmidrule(lr){9-12}
 &  & BEV & Planner & 1s & 2s & 3s & Avg. & 1s & 2s & 3s & Avg. \\
\midrule
ST-P3 & - & - & - & 1.33 & 2.11 & 2.90 & 2.11 & 0.23 & 0.62 & 1.27 & 0.71 \\
UniAD~\cite{UniAD} & - & - & - & 0.48 & 0.96 & 1.65 & 1.03 & 0.05 & 0.17 & 0.71 & 0.31 \\
UniAD & - & \checkmark & \checkmark & 0.20 & 0.42 & 0.75 & 0.46 & 0.02 & 0.25 & 0.84 & 0.37 \\
VAD-Base~\cite{VAD} & - & - & - & 0.69 & 1.22 & 1.83 & 1.25 & 0.06 & 0.68 & 2.52 & 1.09 \\
VAD-Base & - & \checkmark & - & 0.41 & 0.70 & 1.06 & 0.72 & 0.04 & 0.43 & 1.15 & 0.54 \\
VAD-Base & - & \checkmark & \checkmark & 0.17 & 0.34 & 0.60 & 0.37 & 0.04 & 0.27 & 0.67 & 0.33 \\
\midrule
Ego-MLP~\cite{EgoMLP} & - & - & \checkmark & 0.15 & 0.32 & 0.59 & 0.35 & 0.00 & 0.27 & 0.85 & 0.37 \\
BEV-Planner~\cite{BEVPlanner} & - & \checkmark & - & 0.30 & 0.52 & 0.83 & 0.55 & 0.10 & 0.37 & 1.30 & 0.59 \\
BEV-Planner++ & - & \checkmark & \checkmark & 0.16 & 0.32 & 0.57 & 0.35 & 0.00 & 0.29 & 0.73 & 0.34 \\
\midrule
DriveVLM$^{\dagger}$~\cite{DriveVLM} & \checkmark & - & - & 0.18 & 0.34 & 0.68 & 0.40 & 0.10 & 0.22 & 0.45 & 0.27 \\
DriveVLM-Dual~\cite{DriveVLM} & \checkmark & \checkmark & \checkmark & 0.15 & 0.29 & 0.48 & 0.31 & 0.05 & 0.08 & 0.17 & 0.10 \\
OmniDrive$^{\ddagger}$~\cite{OmniDrive} & \checkmark & - & - & 1.15 & 1.96 & 2.84 & 1.98 & 0.80 & 3.12 & 7.46 & 3.79 \\
OmniDrive & \checkmark & - & \checkmark & 0.40 & 0.80 & 1.32 & 0.84 & 0.04 & 0.46 & 2.32 & 0.94 \\
OmniDrive++ & \checkmark & \checkmark & \checkmark & 0.14 & 0.29 & 0.55 & 0.33 & 0.00 & 0.13 & 0.78 & 0.30 \\
Senna~\cite{Senna} & \checkmark & - & - & 0.37 & 0.54 & 0.86 & 0.59 & 0.09 & 0.12 & 0.33 & 0.18 \\
Senna & \checkmark & \checkmark & \checkmark & \textbf{0.11} & \textbf{0.21} & \textbf{0.35} & \textbf{0.22} & \textbf{0.04} & \textbf{0.08} & \textbf{0.13} & \textbf{0.08} \\
EMMA$^{\dagger}$~\cite{EMMA} & \checkmark & - & - & 0.14 & 0.29 & 0.54 & 0.32 & - & - & - & - \\
ORION & \checkmark & \checkmark & - & 0.17 & 0.31 & 0.55 & 0.34 & 0.05 & 0.25 & 0.80 & 0.37 \\
\midrule
\textbf{SmartAD(ours)} & \checkmark & \checkmark & - & \\
\bottomrule
\end{tabular}
\end{table*}

